MELA: Multilingual Evaluation of Linguistic Acceptability

In this work, we present the largest benchmark to date on linguistic acceptability: Multilingual Evaluation of Linguistic Acceptability -- MELA, with 46K samples covering 10 languages from a diverse set of language families. We establish LLM baselines on this benchmark, and investigate cross-lingual transfer in acceptability judgements with XLM-R. In pursuit of multilingual interpretability, we conduct probing experiments with fine-tuned XLM-R to explore the process of syntax capability acquisition. Our results show that GPT-4o exhibits a strong multilingual ability, outperforming fine-tuned XLM-R, while open-source multilingual models lag behind by a noticeable gap. Cross-lingual transfer experiments show that transfer in acceptability judgment is non-trivial: 500 Icelandic fine-tuning examples lead to 23 MCC performance in a completely unrelated language -- Chinese. Results of our probing experiments indicate that training on MELA improves the performance of XLM-R on syntax-related tasks. Our data is available at https://github.com/sjtu-compling/MELA.

==> sec6-mft.tex <==




\section{Multilingual Fine-tuning with Linguistic Acceptability}\label{sec:MFT}
In the previous two sections, we investigated the transfer of linguistic acceptability with both LLMs and supervised XLM-R, and found that in-language training data or in-context examples play a key role in learning linguistic acceptability. To further assess the importance of in-language data, we experiment with training on multiple languages.
To compensate for the impact of training set size, we first downsample data in all languages to the same amount, and then finetune XLM-R on different combinations of languages. Training details are provided in Appendix~\ref{sec:appendix-training}.


\subsection{Experimental Setting}
We downsample sentences in each language to the same number, and train XLM-R in three settings: 1) in-language finetuning; 2) all-language finetuning, where the model is trained on a mixture of data containing an equal number of sentences from ten languages; and 3) all-but-in-language finetuning, where the model is trained on a mixture of data containing an equal number of sentences from nine languages, except the one being evaluated on. 

\subsection{Results}
The results on validation sets in all 10 languages are plotted in Figure~\ref{fig:mft}. When trained and evaluated on the same language, the model's performance scales smoothly with the number of training samples. When trained on sentences from other nine languages, however, the performance saturates at around 500-1000 training samples, consistent with previous findings about multi-task finetuning~\citep{2022SuperNatural}. When trained on all ten languages, the performance scales more steadily than all-but-in-language training, but still lags behind in-language training by a large margin, indicating the importance of in-language training data.


